Visualization of Linear Operations in the Spherical Harmonics Domain

Linear operations on coefficients in the spherical harmonics (SH) transform domain that again yield SH-domain coefficients are an important toolset in many disciplines of research and engineering. They comprise rotations, spatially selective filters, and many other modifications for various applications, or describe the response of a MIMO system to an excitation. It is of particular importance to characterize these operations both qualitatively and quantitatively, and make them accessible for people to work with. In this paper, we identify different key properties of such operations and propose a method for their visualization. With our proposed method, we succeed to show many important aspects of an operation in a single plot and give rise to a comprehensive interpretation of the behavior of a system. In our evaluation, we show the potential of the proposed method on the basis of various practical examples from spatial audio signal processing, where SH-domain filtering is used to modify acoustic scenes given by higher-order Ambisonics signals.

==> figures-data/transformation_nr_dp.tex <==
\newcommand{\datafile}{\figuredatadir/transformation_nr_dp.png}%
\newcommand{\lowerclim}{0.000000}%
\newcommand{\upperclim}{0.774302}%


==> figures-data/transformation_nr_mbf.tex <==
\newcommand{\datafile}{\figuredatadir/transformation_nr_mbf.png}%
\newcommand{\lowerclim}{0.000000}%
\newcommand{\upperclim}{0.930651}%


==> figures-data/transformation_rot.tex <==
\newcommand{\datafile}{\figuredatadir/transformation_rot.png}%
\newcommand{\lowerclim}{0.000000}%
\newcommand{\upperclim}{1.000000}%


==> figures-data/transformation_warp.tex <==
\newcommand{\datafile}{\figuredatadir/transformation_warp.png}%
\newcommand{\lowerclim}{0.000000}%
\newcommand{\upperclim}{0.940065}%


==> tikzlibraryiksblockdiagrams.code.tex <==
%% About this library:
%% This library has been taken from pgflibraryindsigflow.code.tex (which was part of the thesis template) and modified in 2014-09.
%
%% DISCLAIMER: I'm not sure about the differences between pgflibrary and tikzlibrary, but I feel that tikzlibrary fits better here. (This is also valid for \pgfkeys vs. \tikzset)
%
%% Example:
% \usetikzlibrary{iksblockdiagrams}
% ...
% \node (mic) [microphone] {};
% \node (plus) [right=of mic,sumbox] {} %% or use \node[minus above left/..., sumbox];
% 	edge[draw,<-] node [above,signminus,very near start, yshift=2mm] {} (mic);
% \node (speaker) [speaker, right=of plus] {}
% 	edge[draw,<-] (plus);
%%
%% Styles this file provides (not complete):
%%	iks block:
%%		base of (nearly) all the following styles.
%%		Should be used for custom blocks (e.g., filters) as well.
%%	sigempty:
%%		empty circle that can contain a plus sign, multiplication sign, ...
%%		However, like all shapes, it is not drawn by default. Instead, operatorempty should be used.
%%	operatorbox:
%%		meta style that should be applied to some of these shapes, making them the same width, ...
%%	operatorempty:
%%		= sigempty + operatorbox: this should be used to get an empty circle.
%%	sigplus:
%%		shape of a plus sign
%%	sumbox:
%%		operatorbox containing a plus sign
%%	productbox:
%%		operatorbox containing a multiplication sign (sigtimes)
%%	divisionbox:
%%		operatorbox containing a division sign (sigdivide)
%%		Use with care! It will probably not be clear which signal is divided by which.
%%	niceminus (signminus):
%%		minus sign that can be placed at an edge leading to a sumbox: [very near end, yshift=2mm]
%%	dot:
%%		connect two lines using this dot (dotshape)
%%	onoff:
%%		a switch with arbitrary angle and two connectors
%%	sinebox:
%%		operatorbox containing a sine wave (sine)
%%	speaker:
%%		loudspeaker symbol (speakershape)
%%	microphone:
%%		microphone symbol (microphoneshape)
%%	simplerect:
%%		simple rectangle/square
%%	
%%	Additional symbols:
%%	-	DA converter, AD converter, ...
%%	-	bandpass/highpass/lowpass
%%
%%
%% Additionally, macros for easily creating block diagrams of convolutional encoders are given
%%
%% TODO: maybe add a "delaybox"
%% TODO: maybe set dot size to \pgflinewidth (+\pgflinewidth)
%% TODO: rename "sigXXX" to "XXXshape" or "shapeXXX"
%
\ifx\@onlypreamble\@notprerr%% are we outside the preamble?
	\PackageWarning{tikz library iksblockdiagrams}{Not loaded in the preamble. Tikz libraries should NOT be loaded inside a scope, as is produces weird bugs!}%
\fi%
\ifdefined\iksblockdiagrams@loadedlibrary%
	%\PackageWarning{tikz libary iksblockdiagrams}{Test}%
	\endinput%% do not load this twice
	%% NOTE: this does not occur, as tikz does not load a library twice. However, it produces bugs, if the library is loaded inside a scope.
\fi%
\ProvidesFile{tikzlibraryiksblockdiagrams.code.tex}[]%
\def\iksblockdiagrams@loadedlibrary{}%
%\global\def\iksblockdiagrams@loadedlibraryglobal{}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Old "sig" settings
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\pgfkeys{/sig/.cd,
	%% not sure how to use these...
	operator/.style={fill=white,line width=.75pt},
	sigarrow/.style={>=sig},
	default style/.style={line width=0.5pt,/sig/sigarrow},
	transfer/.style={/sig/operator,shape=rectangle,draw,minimum size=0.8cm},
}%
\pgfkeys{/sig/.cd,
	%% not sure how to use these...
	radius/.initial=0.5em, %% old
	%% Needed for the minus sign:
	length/.initial=0.3em,
	vertical sep/.initial=0.3em,
	horizontal sep/.initial=0.25em,
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Common settings for all blocks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{
	iks block/.prefix style={
		%% This style is applied to all items here and should be applied to all custom blocks in your block diagram.
		%% Purpose: have a common style that can be changed, e.g.: iks block/.prefix style={thick, rounded corners}
		%% TODO: apply and test this style with [delay] and [mux]!
		draw,
		minimum width=3em,
		minimum height=2em,
		text height=2ex,
		text depth=0.5ex,
		inner xsep=1ex,%% a bit more
		align=center,
		multiline/.prefix style={text height=,text depth=},%% reset to default
	},
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% New settings for +, ×, /, -
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% taken from pgflibraryindsigflow.code.tex
\tikzset{
	%width/.initial=5mm,
	width/.initial=1.5em,
	dot size/.initial=0.2em,
	sign scale/.initial=0.6,
	operatorbox/.prefix style={
		iks block,
		draw,
		fill/.initial=white,
		width=1.5em,
		line cap=round, %% looks better
	}%
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Settings for microphone and speaker
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{text sep/.initial={1ex}}%
% \tikzset{micradius/.initial={3.5mm}}%
%\tikzset{speaker width/.initial={7mm}}%% == 2·micradius → same width
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Empty node as template for sigplus, ...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%
\newcommand*{\inheritanchors}[1][]{
	\inheritanchor[#1]{north}
	\inheritanchor[#1]{north west}
	\inheritanchor[#1]{north east}
	\inheritanchor[#1]{center}
	\inheritanchor[#1]{west}
	\inheritanchor[#1]{east}
	\inheritanchor[#1]{mid}
	\inheritanchor[#1]{mid west}
	\inheritanchor[#1]{mid east}
	\inheritanchor[#1]{base}
	\inheritanchor[#1]{base west}
	\inheritanchor[#1]{base east}
	\inheritanchor[#1]{south}
	\inheritanchor[#1]{south west}
	\inheritanchor[#1]{south east}
}%
%
\tikzset{operatorempty/.style={sigempty,operatorbox}}%,font=\large %% wrapper for the shape to automatically apply styles
%% Can also be used for custom symbols: \node [operatorempty] {?};
\pgfdeclareshape{sigempty}{
	%% by SZ 2014-09
	\inheritsavedanchors[from=circle] %% has to be before \saveddimen
	\saveddimen\radius{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=circle]
	\inheritanchors[from=circle]
	\inheritbackgroundpath[from=circle]
	%\pgfusepath{fill,stroke}
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Summation node
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \tikzset{sumbox/.style={sigplus,line cap=round}}
\tikzset{sumbox/.style={sigplus,operatorbox}} %% wrapper for the shape to automatically apply styles
\pgfdeclareshape{sigplus}{
	%% by SZ 2014-09
	\inheritsavedanchors[from=sigempty] %% has to be before \saveddimen
	\saveddimen\radius{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=sigempty]
	\inheritanchors[from=sigempty]
	\inheritbackgroundpath[from=sigempty]
	%% Inner path:
	\beforebackgroundpath{
		%% Draw the circle:
		%\pgfutil@tempdima=\radius%% Radius
		%\pgfpathcircle{\centerpoint}{\pgfutil@tempdima}\pgfusepathqstroke%
		%% Draw the sign:
		\pgfmathsetlength{\pgfutil@tempdimb}{\pgfkeysvalueof{/tikz/sign scale}*\radius}%% Size of sign
		\centerpoint%
		\pgf@xa=\pgf@x%
		\pgf@ya=\pgf@y%
		\def\center{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathmoveto{\pgfpointadd{\center}{\pgfqpointpolar{90}{\pgfutil@tempdimb}}}
		\pgfpathlineto{\pgfpointadd{\center}{\pgfqpointpolar{-90}{\pgfutil@tempdimb}}}
		\pgfusepathqstroke%
		\pgfpathmoveto{\pgfpointadd{\center}{\pgfqpointpolar{180}{\pgfutil@tempdimb}}}
		\pgfpathlineto{\pgfpointadd{\center}{\pgfqpointpolar{0}{\pgfutil@tempdimb}}}
		\pgfusepathqstroke%
	}
	
	\nodeparts{} %% no text
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Multiplication node
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\tikzset{productbox/.style={sigtimes,line cap=round}}
\tikzset{productbox/.style={sigtimes,operatorbox}} %% wrapper for the shape to automatically apply styles
\pgfdeclareshape{sigtimes}{
	%% by SZ 2014-09
	\inheritsavedanchors[from=sigempty] %% has to be before \saveddimen
	\saveddimen\radius{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=sigempty]
	\inheritanchors[from=sigempty]
	\inheritbackgroundpath[from=sigempty]
	%% Inner path:
	\beforebackgroundpath{
		%\pgfutil@tempdima=\radius%
		%\pgfpathcircle{\centerpoint}{\pgfutil@tempdima}\pgfusepathqstroke%
		%% Draw the sign:
		\pgfmathsetlength{\pgfutil@tempdimb}{\pgfkeysvalueof{/tikz/sign scale}*\radius}%% Size of sign
		\centerpoint%
		\pgf@xa=\pgf@x%
		\pgf@ya=\pgf@y%
		\def\center{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathmoveto{\pgfpointadd{\center}{\pgfqpointpolar{135}{\pgfutil@tempdimb}}}
		\pgfpathlineto{\pgfpointadd{\center}{\pgfqpointpolar{-45}{\pgfutil@tempdimb}}}
		\pgfusepathqstroke%
		\pgfpathmoveto{\pgfpointadd{\center}{\pgfqpointpolar{-135}{\pgfutil@tempdimb}}}
		\pgfpathlineto{\pgfpointadd{\center}{\pgfqpointpolar{45}{\pgfutil@tempdimb}}}
		\pgfusepathqstroke%
	}
	
	\nodeparts{} %% no text
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Division node
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\tikzset{divisionbox/.style={sigdivide,line cap=round}}
% \tikzset{divisionbox/.style={ %% wrapper for the shape to automatically apply styles
% 		sigdivide, %% obviously needed
% 		draw,
% 		fill=white,
% 		width=1em,
% 		line cap=round, %% looks better
% 	}}%
\tikzset{divisionbox/.style={sigdivide,operatorbox}} %% wrapper for the shape to automatically apply styles
\pgfdeclareshape{sigdivide}{
	%% by SZ 2014-09
	\inheritsavedanchors[from=sigempty] %% has to be before \saveddimen
	\saveddimen\radius{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=sigempty]
	\inheritanchors[from=sigempty]
	\inheritbackgroundpath[from=sigempty]
	%% Inner path:
	\beforebackgroundpath{
		% \pgfutil@tempdima=\radius%
		% \pgfpathcircle{\centerpoint}{\pgfutil@tempdima}\pgfusepathqstroke%
		%% Draw the sign:
		\pgfmathsetlength{\pgfutil@tempdimb}{\pgfkeysvalueof{/tikz/sign scale}*\radius}%% Size of sign
		\centerpoint%
		\pgf@xa=\pgf@x%
		\pgf@ya=\pgf@y%
		\def\center{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathmoveto{\pgfpointadd{\center}{\pgfqpointpolar{-135}{\pgfutil@tempdimb}}}
		\pgfpathlineto{\pgfpointadd{\center}{\pgfqpointpolar{45}{\pgfutil@tempdimb}}}
		\pgfusepathqstroke%
	}
	
	\nodeparts{} %% no text
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Minus sign node
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% This is NOT intended as a subtraction node, but it is just the minus that can be set, e.g., "very near end, yshift=2mm", on an edge.
%\tikzset{niceminus/.style={signminus,line cap=round}}
\tikzset{niceminus/.style={ %% wrapper for the shape to automatically apply styles
		signminus, %% obviously needed
		draw,
		%fill=white,
		line cap=round, %% looks better
	}}%
\pgfdeclareshape{signminus}{
	%% taken from pgflibraryindsigflow.code.tex, edited by sz since 2014-09
	
	\savedanchor\centerpoint{%
		\pgfpointorigin%
	}
	\savedanchor\leftedge{
		\pgfpointadd{\pgfpointorigin}{\pgfpointscale{-0.5}{\pgfpoint{\pgfkeysvalueof{/sig/length}}{0pt}}}
	}
	\savedanchor\rightedge{
		\pgfpointadd{\pgfpointorigin}{\pgfpointscale{0.5}{\pgfpoint{\pgfkeysvalueof{/sig/length}}{0pt}}}
	}
	
	\saveddimen\signwidth{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/sig/length}}%
	}
	
	\anchor{center}{\centerpoint}
	\anchor{north}{\centerpoint}
	\anchor{west}{\pgfpointadd{\leftedge}{\pgfpoint{-\pgfkeysvalueof{/sig/horizontal sep}}{\pgfkeysvalueof{/sig/vertical sep}}}}
	\anchor{east}{\rightedge}
	\anchor{north west}{\leftedge}
	\anchor{north east}{\rightedge}
	\anchor{mid}{\centerpoint}
	\anchor{mid west}{\leftedge}
	\anchor{mid east}{\rightedge}
	\anchor{base}{\centerpoint}
	\anchor{base west}{\leftedge}
	\anchor{base east}{\rightedge}
	\anchor{south}{\centerpoint}
	\anchor{south west}{\leftedge}
	\anchor{south east}{\rightedge}
	\anchorborder{\centerpoint}
	
	\backgroundpath{
		\pgfsetarrows{-}
		\leftedge 	\pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
		\rightedge	\pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
		\pgfusepathqstroke %% draw it by default
	}
	
	\nodeparts{} %% no text
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Minus sign placements
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Usage:
% \node[sumbox,minus above left];
%% or
% \draw ... node[sumbox,minus below right={thick,blue}];
%% It might also be useful to say \tikzset{niceminus/.append style={thick}}
%
\tikzset{
	minus helper/.style={prefix after command={\pgfextra{%
				\let\tikzlastnode@fixed\tikzlastnode%%% see http://tex.stackexchange.com/a/213815/50960
				\def\minus@xoffset{1mm}%% This could be a global macro
				\def\minus@yoffset{1mm}%% This could be a global macro
				\def\minus@siglen{\pgfkeysvalueof{/sig/length}}%% This might be a global macro
			}}},
	minus above left/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.north) ++(-0.5*\minus@siglen,0) ++(-\minus@xoffset,\minus@yoffset) node[niceminus,#1] {};
			}}},
	minus above right/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.north) ++(0.5*\minus@siglen,0) ++(\minus@xoffset,\minus@yoffset) node[niceminus,#1] {};
			}}},
	minus below left/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.south) ++(-0.5*\minus@siglen,0) ++(-\minus@xoffset,-\minus@yoffset) node[niceminus,#1] {};
			}}},
	minus below right/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.south) ++(0.5*\minus@siglen,0) ++(\minus@xoffset,-\minus@yoffset) node[niceminus,#1] {};
			}}},
	minus right above/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.east) ++(0.5*\minus@siglen,0) ++(\minus@xoffset,\minus@yoffset) node[niceminus,#1] {};
			}}},
	minus right below/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.east) ++(0.5*\minus@siglen,0) ++(\minus@xoffset,-\minus@yoffset) node[niceminus,#1] {};
			}}},
	minus left above/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.west) ++(-0.5*\minus@siglen,0) ++(-\minus@xoffset,\minus@yoffset) node[niceminus,#1] {};
			}}},
	minus left below/.style={minus helper,append after command={\pgfextra{
				\path (\tikzlastnode@fixed.west) ++(-0.5*\minus@siglen,0) ++(-\minus@xoffset,-\minus@yoffset) node[niceminus,#1] {};
			}}},
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sine wave
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{sinebox/.style={sine,operatorbox}}%% wrapper for the shape to automatically apply styles
\pgfdeclareshape{sine}{
	%% by SZ 2014-11
	\inheritsavedanchors[from=sigempty] %% has to be before \saveddimen
	\saveddimen\radius{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=sigempty]
	\inheritanchors[from=sigempty]
	\inheritbackgroundpath[from=sigempty]
	%% Inner path:
	\beforebackgroundpath{
		%% Draw the circle:
		%\pgfutil@tempdima=\radius%% Radius
		%\pgfpathcircle{\centerpoint}{\pgfutil@tempdima}\pgfusepathqstroke%
		%% Draw the sign:
		\pgfmathsetlength{\pgfutil@tempdimb}{\pgfkeysvalueof{/tikz/sign scale}*\radius}%% Size of sign
		\centerpoint%
		\pgf@xa=\pgf@x%
		\pgf@ya=\pgf@y%
		\def\center{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathmoveto{\pgfpointadd{\center}{\pgfqpointpolar{180}{\pgfutil@tempdimb}}}
		%
		\pgf@xb=\pgfutil@tempdimb %% half "wavelength"
		\divide \pgf@xb by 2
		\pgf@yb=\pgfutil@tempdimb %% amplitude
		\divide \pgf@yb by 2
		\pgfpathsine{\pgfqpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathcosine{\pgfqpoint{\pgf@xb}{-\pgf@yb}}
		\pgfpathsine{\pgfqpoint{\pgf@xb}{-\pgf@yb}}
		\pgfpathcosine{\pgfqpoint{\pgf@xb}{\pgf@yb}}
		% \pgfpathsine{\pgfpointadd{\center}{\pgfqpointpolar{45}{\pgfutil@tempdimb}}}
		% \pgfpathcosine{\pgfpointadd{\center}{\pgfqpointpolar{-45}{\pgfutil@tempdimb}}}
		% \pgfpathsine{\pgfpointadd{\center}{\pgfqpointpolar{-45}{\pgfutil@tempdimb}}}
		% \pgfpathcosine{\pgfpointadd{\center}{\pgfqpointpolar{45}{\pgfutil@tempdimb}}}
		\pgfusepathqstroke%
	}
	
	\nodeparts{} %% no text
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% "sig" arrow
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% TODO: make the size adjustable
%% taken from pgflibraryindsigflow.code.tex (size was 0.3pt), edited by sz since 2014-09
\pgfarrowsdeclare{sig}{sig}{
	%% Extend code:
	\pgfutil@tempdima=0.2pt%
	\advance\pgfutil@tempdima by.25\pgflinewidth%
	\pgfutil@tempdimb=8.705\pgfutil@tempdima\advance\pgfutil@tempdimb by.5\pgflinewidth%
	\pgfarrowsleftextend{+-\pgfutil@tempdimb}
	\pgfutil@tempdimb=.5\pgfutil@tempdima\advance\pgfutil@tempdimb by1.28\pgflinewidth%
	\pgfarrowsrightextend{+\pgfutil@tempdimb}
}{
	%% Arrow tip code:
	\pgfutil@tempdima=0.2pt%
	\advance\pgfutil@tempdima by.25\pgflinewidth%
	\pgfsetdash{}{+0pt}
	\pgfsetmiterjoin
	\pgfpathmoveto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{158}{10\pgfutil@tempdima}}}
	\pgfpathlineto{\pgfqpoint{0.5\pgfutil@tempdima}{0\pgfutil@tempdima}}
	\pgfpathlineto{\pgfpointadd{\pgfqpoint{0.5\pgfutil@tempdima}{0pt}}{\pgfqpointpolar{-158}{10\pgfutil@tempdima}}}
	\pgfpathclose
	\pgfusepathqfillstroke
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% dot connector
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{dot/.style={dotshape,draw,fill}} %% draw might not be used
\tikzset{empty dot/.style={dotshape,draw,fill,dot inner color=white}} %% draw might not be used
\tikzset{dot inner color/.initial=none}
\pgfdeclareshape{dotshape}{ %% this is just a dot
	%% by SZ 2014-09
	%% The dot size is "relative" to the line width, i.e., it denotes the amount by which it is larger than the line
	\inheritsavedanchors[from=circle] %% has to be before \saveddimen
	\saveddimen\radius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/dot size}}
		\advance\pgf@x by \pgflinewidth
		\divide\pgf@x by 2
	}
	\saveddimen\radius@nolinewidth{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/dot size}}
		%\advance\pgf@x by 0.5\pgflinewidth
		\divide\pgf@x by 2
	}
	\saveddimen\sqrt@two@radius{%
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/dot size}}
		%\advance\pgf@x by \pgflinewidth
		\divide\pgf@x by 2
		\multiply\pgf@x by 1000
		\divide\pgf@x by 1414
	}
	
	\anchorborder{\centerpoint}
	\anchor{center}{\centerpoint}
	\anchor{base}{\centerpoint}
	\anchor{north}{\centerpoint\advance\pgf@y by\radius\advance\pgf@y by -0.5\pgflinewidth}
	\anchor{south}{\centerpoint\advance\pgf@y by-\radius\advance\pgf@y by 0.5\pgflinewidth}
	\anchor{west}{\centerpoint\advance\pgf@x by-\radius\advance\pgf@x by 0.5\pgflinewidth}
	\anchor{east}{\centerpoint\advance\pgf@x by\radius\advance\pgf@x by -0.5\pgflinewidth}
	\anchor{north west}{\centerpoint\advance\pgf@x by-\sqrt@two@radius\advance\pgf@y by\sqrt@two@radius}
	\anchor{south west}{\centerpoint\advance\pgf@x by-\sqrt@two@radius\advance\pgf@y by-\sqrt@two@radius}
	\anchor{north east}{\centerpoint\advance\pgf@x by\sqrt@two@radius\advance\pgf@y by\sqrt@two@radius}
	\anchor{south east}{\centerpoint\advance\pgf@x by\sqrt@two@radius\advance\pgf@y by-\sqrt@two@radius}
	
	\anchorborder{ %% from pgfmoduleshapes.code.tex
		\pgf@xa=\pgf@x%
		\pgf@ya=\pgf@y%
		\edef\pgf@marshal{%
			\noexpand\pgfpointborderellipse
			{\noexpand\pgfqpoint{\the\pgf@xa}{\the\pgf@ya}}
			{\noexpand\pgfqpoint{\radius@nolinewidth}{\radius@nolinewidth}}%
		}%
		\pgf@marshal%
		\pgf@xa=\pgf@x%
		\pgf@ya=\pgf@y%
		\centerpoint%
		\advance\pgf@x by\pgf@xa%
		\advance\pgf@y by\pgf@ya%
	}
	
	
	\inheritbackgroundpath[from=circle]
	%\pgfusepathqfillstroke
	\backgroundpath{ %% new since 2014-12
		\pgfutil@tempdima=\radius%
		\pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
		\pgfusepathqfill %% only fill, no stroke: do not draw the line
		%\pgfusepathqfillstroke
		%
		%% if an inner color is defined (i.e., not "none"), draw an inner circle with that color:
		\edef\temp{\pgfkeysvalueof{/tikz/dot inner color}}
		\def\none{none}
		\ifx\temp\none\else
			\advance \pgfutil@tempdima by -\pgflinewidth
			\pgfpathcircle{\centerpoint}{\pgfutil@tempdima}%
			\pgfsetcolor{\pgfkeysvalueof{/tikz/dot inner color}}
			\pgfusepathqfill %% only fill, no stroke: do not draw the line
		\fi
	}
	
	\nodeparts{} %% no text
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% on/off switch
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{onoff/.style={onoffswitchshape,draw,fill,width=5mm,line cap=round,anchor=in}}%
\tikzset{
	switch angle/.initial=15,
	in dot inner color/.initial=none,
	out dot inner color/.initial=none,
}%
\pgfdeclareshape{onoffswitchshape}{%% This is a switch
	%% by SZ 2014-11
	%% The distance between both connectors can be specified with [width=...] (default: 5mm).
	%% The angle (in degree) of the switch can be defined with [switch angle=...] (default: 15).
	%% Angle around 0 (-90...+90): connected to the left (in) connector
	%% Angle around 360 (270...450): connected to the right (out) connector
	%
	%% Anchors:
	\savedanchor\centerpoint{%
		%% Standard things:
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by-.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\inpoint{%
		%% input (left) connector
		%% Standard things:
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by-.5\dp\pgfnodeparttextbox%
		%% go left
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/tikz/width}}
		\advance\pgf@x by -.5\pgf@xc
	}
	\savedanchor\outpoint{%
		%% output (right) connector
		%% Standard things:
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by-.5\dp\pgfnodeparttextbox%
		%% go right
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/tikz/width}}
		\advance\pgf@x by .5\pgf@xc
	}
	\savedanchor\switchinpoint{%
		%% input of switch line
		%% Standard things:
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by-.5\dp\pgfnodeparttextbox%
		%% Get settings:
		\pgfmathsetmacro{\switchangle}{\pgfkeysvalueof{/tikz/switch angle}}
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/tikz/width}}
		%% Draw
		\pgfmathtruncatemacro{\switchangletemp}{\switchangle>0?1:-1}%% \ifnum only can use integers
		\ifnum\switchangletemp<0%
			%% go right
			\advance\pgf@x by .5\pgf@xc
			%% make rotation:
			\pgfmathsetlength{\pgf@xb}{\pgf@xc*cos(\switchangle)}
			\pgfmathsetlength{\pgf@yb}{\pgf@xc*sin(\switchangle)}
			\advance\pgf@x by -\pgf@xb
			\advance\pgf@y by \pgf@yb
		\else
			% go left
			\advance\pgf@x by -.5\pgf@xc
		\fi
	}
	\savedanchor\switchoutpoint{%
		%% input of switch line
		%% Standard things:
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by-.5\dp\pgfnodeparttextbox%
		%% Get settings:
		\pgfmathsetmacro{\switchangle}{\pgfkeysvalueof{/tikz/switch angle}}
		\pgfmathsetlength\pgf@xc{\pgfkeysvalueof{/tikz/width}}
		%% Draw
		\pgfmathtruncatemacro{\switchangletemp}{\switchangle>0?1:-1}%% \ifnum only can use integers
		\ifnum\switchangletemp>0%
			%% go left
			\advance\pgf@x by -.5\pgf@xc
			%% make rotation:
			\pgfmathsetlength{\pgf@xb}{\pgf@xc*cos(180-\switchangle)}
			\pgfmathsetlength{\pgf@yb}{\pgf@xc*sin(180-\switchangle)}
			\advance\pgf@x by -\pgf@xb
			\advance\pgf@y by \pgf@yb
		\else
			% go right
			\advance\pgf@x by .5\pgf@xc
		\fi
	}
	\saveddimen\dotradius{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/dot size}}
		\advance\pgf@x by \pgflinewidth %% TODO: check the desired behaviour also in "dot"
		\divide\pgf@x by 2
	}
	\saveddimen\halfwidth{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	
	%\anchorborder{\inpoint} %% TODO: improve!
	\anchorborder{
		%% TODO: check this!
		\ifdim\pgf@x>0pt
			\outpoint
		\else
			\inpoint
		\fi
	}
	%% actually, the center does not make sense:
	%\anchor{center}{\inpoint \advance \pgf@x by -\dotradius} %??
	\anchor{center}{\centerpoint}%% this should be the center. Just set another default anchor, if the following is desired:
	%\anchor{center}{\inpoint}%% This is not the center, but the switch should "start" at this point when drawn
	\anchor{realcenter}{\centerpoint}
	\anchor{base}{\inpoint}
	\anchor{north}{\switchinpoint} %% might not be the best idea
	\anchor{south}{\switchoutpoint} %% might not be the best idea
	%% useful points:
	\anchor{west}{\inpoint}
	\anchor{east}{\outpoint}
	\anchor{in}{\inpoint}
	\anchor{out}{\outpoint}
	% \anchor{north west}{\centerpoint}
	% \anchor{south west}{\centerpoint}
	% \anchor{north east}{\centerpoint}
	% \anchor{south east}{\centerpoint}
	
	%\inheritbackgroundpath[from=circle]
	\backgroundpath{
		\pgfutil@tempdima=\dotradius%
		
		\pgfpathmoveto{\switchinpoint}
		\pgfpathlineto{\switchoutpoint}
		\pgfusepathqfillstroke
		
		%% Draw both connector dots:
		\pgfpathcircle{\inpoint}{\pgfutil@tempdima}%
		\pgfpathcircle{\outpoint}{\pgfutil@tempdima}%
		\pgfusepathqfill %% stroke
		
		%% Fill both connector dots if desired:
		\advance \pgfutil@tempdima by -\pgflinewidth
		\def\none{none}
		%
		\edef\temp{\pgfkeysvalueof{/tikz/in dot inner color}}
		\ifx\temp\none\else
			\pgfpathcircle{\inpoint}{\pgfutil@tempdima}%
			\pgfsetcolor{\pgfkeysvalueof{/tikz/in dot inner color}}
			\pgfusepathqfill %% only fill, no stroke: do not draw the line
		\fi
		\edef\temp{\pgfkeysvalueof{/tikz/out dot inner color}}
		\ifx\temp\none\else
			\pgfpathcircle{\outpoint}{\pgfutil@tempdima}%
			\pgfsetcolor{\pgfkeysvalueof{/tikz/out dot inner color}}
			\pgfusepathqfill %% only fill, no stroke: do not draw the line
		\fi
	}
	\nodeparts{} %% no text
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Microphone:
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{microphone/.style={ %% wrapper for the shape to automatically apply styles
		microphoneshape, %% obviously needed
		iks block,
		fill=white,
		line cap=round, %% looks better
	}}%
\pgfdeclareshape{microphoneshape}{
	%% by SZ 2014-09
	%% Note: The node text should not be used. It might be ignored in future releases.
	
	%% Options:
	\saveddimen\radius{
		%\pgf@x=\pgfkeys{/tikz/micradius/.get=\radius}
		\pgfmathsetlength{\pgf@x}{\pgfkeysvalueof{/tikz/width}}% 
		%\pgf@x=\pgf@xa%
		\divide\pgf@x by 2
	}
	
	%% Anchors:
	\savedanchor\centerpoint{%
		\pgfkeys{/tikz/width/.get=\radius}%% cannot use the saveddimen here for some reason
		\pgf@x=.5\wd\pgfnodeparttextbox%% middle
		\pgf@y=\ht\pgfnodeparttextbox%% top
		\pgfkeys{/tikz/text sep/.get=\textsep}
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/text sep}}%
		\expandafter\advance \expandafter\pgf@y by \pgf@xa
		%\expandafter\advance \expandafter\pgf@y by \pgfkeysvalueof{/tikz/text sep}
		\expandafter\advance \expandafter\pgf@y by \radius
		%\advance\pgf@y by -.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\textcenter{%
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by -.5\dp\pgfnodeparttextbox%
	}
	\anchor{textcenter}{\textcenter}
	
	\anchor{center}{\centerpoint}
	\anchor{north}{\centerpoint\advance\pgf@y by\radius}
	\anchor{south}{\centerpoint\advance\pgf@y by-\radius}
	\anchor{west}{\centerpoint\advance\pgf@x by-\radius}
	\anchor{east}{\centerpoint\advance\pgf@x by\radius}
	\anchorborder{\centerpoint\advance\pgf@x by\radius} %% == east
	%\inheritanchor[from=circle]{north west} %% does it make sense?
	%\inheritanchor[from=circle]{south west} %% does it make sense?
	\anchor{north west}{\centerpoint\advance\pgf@x by-\radius\advance\pgf@y by\radius}
	\anchor{south west}{\centerpoint\advance\pgf@x by-\radius\advance\pgf@y by-\radius}
	\inheritanchor[from=circle]{north east}
	\inheritanchor[from=circle]{south east}
	
	%\beforebackgroundpath{
	\backgroundpath{
		%% Circle:
		%\pgfpathcircle{\centerpoint}{\micradius}%% generates a plot stream?!
		\pgfpathcircle{\centerpoint}{\radius}%% generates a plot stream?!
		%% Line:
		\centerpoint \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		\pgfpathmoveto{\pgfpoint{\pgf@xb-\radius}{\pgf@yb+\radius}}
		\pgfpathlineto{\pgfpoint{\pgf@xb-\radius}{\pgf@yb-\radius}}
		% %% Fill
		%% This is now done by the wrapper style
		% \tikz@mode
		% \iftikz@mode@fill
		% 	\pgfusepath{draw,fill}
		% \else
		% 	\pgfusepath{draw}
		% \fi
	}
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Loudspeaker
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{speaker/.style={ %% wrapper for the shape to automatically apply styles
		speakershape, %% obviously needed
		iks block,
		fill=white,
		line cap=round, %% only visible with "rounded corners"
	}}%
\pgfdeclareshape{speakershape}{
	%% by SZ 2014-09
	%% Known issue: the text is not positioned correctly if the size is given in "em".
	%% Note: The node text should not be used. It might be ignored in future releases.
	
	\saveddimen\speakerwidth{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}% 
		\pgf@x=\pgf@xa%
	}
	\saveddimen\speakerunit{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}% 
		\pgf@x=\pgf@xa%
		\divide\pgf@x by 12%
	}
	
	\savedanchor\centerpoint{%
		\pgfkeys{/tikz/width/.get=\speakerwidth}%% cannot use the saveddimen here for some reason
		\pgf@x=.5\wd\pgfnodeparttextbox%% middle
		\pgf@y=\ht\pgfnodeparttextbox%% top
		\pgfkeys{/tikz/text sep/.get=\textsep}
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/text sep}}%
		\expandafter\advance \expandafter\pgf@y by \pgf@xa
		%\expandafter\advance \expandafter\pgf@y by \pgfkeysvalueof{/tikz/text sep}
		\expandafter\advance \expandafter\pgf@y by \speakerwidth
		\pgfutil@tempdima=\speakerwidth \divide \pgfutil@tempdima by 12
		\advance\pgf@x by -6\pgfutil@tempdima
		%\advance\pgf@y by -.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\textcenter{%
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by -.5\dp\pgfnodeparttextbox%
	}
	\anchor{textcenter}{\textcenter}
	
	\anchor{center}{\centerpoint}
	%% TODO: improve these
	\anchor{north}{
		\centerpoint
		\pgfutil@tempdima=\speakerunit
		\advance\pgf@x by 6\pgfutil@tempdima
		\advance\pgf@y by 7\pgfutil@tempdima
	}
	\anchor{south}{
		\centerpoint
		\pgfutil@tempdima=\speakerunit
		\advance\pgf@x by 6\pgfutil@tempdima
		\advance\pgf@y by -7\pgfutil@tempdima
	}
	\anchor{west}{\centerpoint}
	\anchorborder{\centerpoint} %% == west
	\anchor{east}{\centerpoint\advance\pgf@x by \speakerwidth}
	\anchor{north east}{
		\centerpoint
		\pgfutil@tempdima=\speakerunit
		\advance\pgf@x by 12\pgfutil@tempdima
		\advance\pgf@y by 13\pgfutil@tempdima
	}
	\anchor{south east}{
		\centerpoint
		\pgfutil@tempdima=\speakerunit
		\advance\pgf@x by 12\pgfutil@tempdima
		\advance\pgf@y by -13\pgfutil@tempdima
	}
	\anchor{north west}{
		\centerpoint
		\pgfutil@tempdima=\speakerunit
		\advance\pgf@y by 7\pgfutil@tempdima
	}
	\anchor{south west}{
		\centerpoint
		\pgfutil@tempdima=\speakerunit
		\advance\pgf@y by -7\pgfutil@tempdima
	}
	
	\anchor{east}{\centerpoint \advance\pgf@x by \speakerwidth}
	
	%\beforebackgroundpath{
	\backgroundpath{
		%% get and set options
		\pgfutil@tempdima=\speakerunit
		
		%% Calculate points:
		\centerpoint \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\pgf@xb=\pgf@xa \advance\pgf@xb by 6\pgfutil@tempdima
		\pgf@xc=\pgf@xb \advance\pgf@xc by 6\pgfutil@tempdima
		\pgf@yb=\pgf@ya \advance\pgf@yb by 7\pgfutil@tempdima
		\advance\pgf@ya by -7\pgfutil@tempdima
		\pgf@yc=\pgf@yb \advance\pgf@yc by 6\pgfutil@tempdima
		
		
		%% Draw outer shape:
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		\pgf@yc=\pgf@ya \advance\pgf@yc by -6\pgfutil@tempdima
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		%\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathclose %% allow round corners
		%% Inner line:
		\pgfpathmoveto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		
		% %% Fill:
		%% This is now done by the wrapper style
		% \tikz@mode
		% \iftikz@mode@fill
		% 	\pgfusepath{draw,fill}
		% \else
		% 	\pgfusepath{draw}
		% \fi
	}
}%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Simple rectangle as base for bandpass, ...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\pgfdeclareshape{simplerect}{
	%% by SZ 2014-11
	%% Options:
	
	\saveddimen\width{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}% 
		\pgf@x=\pgf@xa%
	}
	\saveddimen\halfwidth{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}% 
		\pgf@x=\pgf@xa%
		\divide \pgf@x by 2
	}
	\saveddimen\smallwidth{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}% 
		\pgf@x=\pgf@xa%
		\divide \pgf@x by 4
	}
	
	\savedanchor\centerpoint{%
		\pgfkeys{/tikz/width/.get=\width}%% cannot use the saveddimen here for some reason
		\pgf@x=.5\wd\pgfnodeparttextbox%% middle
		\pgf@y=2\ht\pgfnodeparttextbox%% top
		\advance\pgf@y by \width
		%\pgf@y=\ht\pgfnodeparttextbox%% top
		%\advance\pgf@y by .5\dp\pgfnodeparttextbox%
		\pgfkeys{/tikz/text sep/.get=\textsep}
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/text sep}}%
		\expandafter\advance \expandafter\pgf@y by \pgf@xa
		%\expandafter\advance \expandafter\pgf@y by \pgfkeysvalueof{/tikz/text sep}
		%\expandafter\advance \expandafter\pgf@y by \width
		%\pgfutil@tempdima=\width \divide \pgfutil@tempdima by 12
		%\advance\pgf@x by -6\pgfutil@tempdima
		%\advance\pgf@y by -.5\dp\pgfnodeparttextbox%
	}
	\savedanchor\textcenter{%
		\pgf@x=.5\wd\pgfnodeparttextbox%
		\pgf@y=.5\ht\pgfnodeparttextbox%
		\advance\pgf@y by -.5\dp\pgfnodeparttextbox%
	}
	\anchor{textcenter}{\textcenter}
	
	\anchor{base}{\centerpoint}
	\anchor{center}{\centerpoint}
	%% TODO: check whether they are correct
	\anchor{north}{\centerpoint \advance\pgf@y by \halfwidth}
	\anchor{south}{\centerpoint \advance\pgf@y by -\halfwidth}
	\anchor{west}{\centerpoint \advance\pgf@x by -\halfwidth}
	\anchor{east}{\centerpoint\advance\pgf@x by \halfwidth}
	\anchor{north east}{\centerpoint\advance\pgf@x by \halfwidth \advance\pgf@y by \halfwidth}
	\anchor{north west}{\centerpoint\advance\pgf@x by -\halfwidth \advance\pgf@y by \halfwidth}
	\anchor{south east}{\centerpoint\advance\pgf@x by \halfwidth \advance\pgf@y by -\halfwidth}
	\anchor{south west}{\centerpoint\advance\pgf@x by -\halfwidth \advance\pgf@y by -\halfwidth}
	%% intermediate points, e.g. for blocks with 2 or 3 inputs
	\anchor{north east east}{\centerpoint\advance\pgf@x by \halfwidth \advance\pgf@y by \smallwidth}
	\anchor{north north east}{\centerpoint\advance\pgf@x by \smallwidth \advance\pgf@y by \halfwidth}
	\anchor{north north west}{\centerpoint\advance\pgf@x by -\smallwidth \advance\pgf@y by \halfwidth}
	\anchor{north west west}{\centerpoint\advance\pgf@x by -\halfwidth \advance\pgf@y by \smallwidth}
	\anchor{south west west}{\centerpoint\advance\pgf@x by -\halfwidth \advance\pgf@y by -\smallwidth}
	\anchor{south south west}{\centerpoint\advance\pgf@x by -\smallwidth \advance\pgf@y by -\halfwidth}
	\anchor{south south east}{\centerpoint\advance\pgf@x by \smallwidth \advance\pgf@y by -\halfwidth}
	\anchor{south east east}{\centerpoint\advance\pgf@x by \halfwidth \advance\pgf@y by -\smallwidth}
	%% Other:
	\anchorborder{\centerpoint} %% Currently it has to be specified manually
	\anchorborder{%% from pgfmoduleshapes.code.tex
		\pgf@xb=\pgf@x% xb/yb is target
		\pgf@yb=\pgf@y%
		% \southwest%
		% \pgf@xa=\pgf@x% xa/ya is se
		% \pgf@ya=\pgf@y%
		%% south west:
		\centerpoint
		\pgf@xa=\pgf@x \advance\pgf@xa by -\halfwidth
		\pgf@ya=\pgf@y \advance\pgf@ya by -\halfwidth
		% \northeast%
		\centerpoint \advance\pgf@y by \halfwidth \advance\pgf@x by \halfwidth %% north east
		\advance\pgf@x by-\pgf@xa%
		\advance\pgf@y by-\pgf@ya%
		\pgf@xc=.5\pgf@x% x/y is half width/height
		\pgf@yc=.5\pgf@y%
		\advance\pgf@xa by\pgf@xc% xa/ya becomes center
		\advance\pgf@ya by\pgf@yc%
		\edef\pgf@marshal{%
			\noexpand\pgfpointborderrectangle
			{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
			{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
		}%
		\pgf@process{\pgf@marshal}%
		\advance\pgf@x by\pgf@xa%
		\advance\pgf@y by\pgf@ya%
	}
	
	\backgroundpath{
		%% get and set options
		\pgfutil@tempdima=\halfwidth
		
		%% Calculate points:
		\centerpoint
		%% south west:
		\pgf@xa=\pgf@x \advance\pgf@xa by -\halfwidth
		\pgf@ya=\pgf@y \advance\pgf@ya by -\halfwidth
		%% north east:
		\pgf@xc=\pgf@x \advance\pgf@xc by \halfwidth
		\pgf@yc=\pgf@y \advance\pgf@yc by \halfwidth
		
		
		%% Draw outer shape:
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yc}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@ya}}
		\pgfpathclose %% allow round corners
		
		% %% Fill:
		%% This is now done by the wrapper style
		% \tikz@mode
		% \iftikz@mode@fill
		% 	\pgfusepath{draw,fill}
		% \else
		% 	\pgfusepath{draw}
		% \fi
	}
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% D/A, A/D, ... converters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% converters that look good everywhere:
\tikzset{AD converter/.style={converter,scaled north west label=A,scaled south east label=D}}%
\tikzset{DA converter/.style={converter,scaled north west label=D,scaled south east label=A}}%
%% converters without scaled text – the text fits to all other text:
\tikzset{unscaled AD converter/.style={converter,north west label=A,south east label=D}}%
\tikzset{unscaled DA converter/.style={converter,north west label=D,south east label=A}}%
%% Gerenal converters:
\tikzset{converter/.style={
		convertershape,
		operatorbox,
		text depth=,text height=,%% undo these settings from [iks block]
		scaled north west label/.initial={~},%% should not be empty! use ~ instead
		scaled south east label/.initial={~},%% should not be empty! use ~ instead
		north west label/.initial={},
		south east label/.initial={},
		label scale/.initial=1,
		converter inner/.prefix style={},%% Usage: [converter inner/.style={inner sep=<value>}]
		minimum width=0,
		minimum height=0,
	}
}%
\pgfdeclareshape{convertershape}{ %% A/D or similar
	%% by SZ 2014-12
	\inheritsavedanchors[from=simplerect] %% has to be before \saveddimen
	\saveddimen\width{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}% 
		\pgf@x=\pgf@xa%
	}
	\saveddimen\halfwidth{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}% 
		\pgf@x=\pgf@xa%
		\divide \pgf@x by 2
	}
	\saveddimen\labelsize{
		\pgfmathsetlength{\pgf@x}{0.8*\pgfkeysvalueof{/tikz/label scale}*\pgfkeysvalueof{/tikz/width}/2}
	}
	\inheritanchorborder[from=simplerect]
	\inheritanchors[from=simplerect]
	\inheritbackgroundpath[from=simplerect]
	
	%% Inner path:
	\beforebackgroundpath{
		%%% Strike through:
		\pgfmathsetlength{\pgfutil@tempdimb}{\width}%
		%% Helper to get the x and y values of rounded corners:
		\ifdefined\pgf@corner@arc
			\def\evaluate@pgf@corner@arc##1##2{
				\pgfmathsetlength{\pgf@xa}{##1*0.29289} %% 0.29289 = 1-cos(π/4)
				\pgfmathsetlength{\pgf@ya}{##2*0.29289} %% Note: might only work for x = y
			}
			\expandafter\evaluate@pgf@corner@arc\pgf@corner@arc %% Note: \pgf@corner@arc is set to 2 tokens; the x value and the y value
		\else
			\pgfmathsetlength{\pgf@xa}{0pt}
			\pgfmathsetlength{\pgf@ya}{0pt}
		\fi
		%% North east:
		\centerpoint \advance\pgf@x by \halfwidth \advance\pgf@y by \halfwidth
		\advance\pgf@x by -\pgf@xa \advance\pgf@y by -\pgf@ya %% adjust for rounded corners
		\pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
		%% South west:
		\centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by -\halfwidth
		\advance\pgf@x by +\pgf@xa \advance\pgf@y by +\pgf@ya %% adjust for rounded corners
		\pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
		\pgfusepathqstroke%
		%%% Add Labels:
		{
			\pgftransformshift{\centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by \halfwidth}
			%\pgfnode{rectangle}{north west}{\pgfkeysvalueof{/tikz/north west label}}{}{}
			\node [rectangle,anchor=north west,inner sep=0.1*\halfwidth,converter inner] {%
					\resizebox{\labelsize}{!}{%
						\pgfkeysvalueof{/tikz/scaled north west label}%% should not be empty! use ~ instead
					}%
				};
			\node [rectangle,anchor=north west,converter inner] {%
					\pgfkeysvalueof{/tikz/north west label}%
				};
		}
		{
			\pgftransformshift{\centerpoint \advance\pgf@x by \halfwidth \advance\pgf@y by -\halfwidth}
			%\pgfnode{rectangle}{south east}{\pgfkeysvalueof{/tikz/south east label}}{}{}
			%
			\node [rectangle,anchor=south east,inner sep=0.1*\halfwidth,converter inner] {%
					\resizebox{\labelsize}{!}{%
						\pgfkeysvalueof{/tikz/scaled south east label}%% should not be empty! use ~ instead
					}%
				};
			\node [rectangle,anchor=south east,converter inner] {%
					\pgfkeysvalueof{/tikz/south east label}%
				};
		}
	}
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Waves for bandpass, ...
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% The following commands need to have the wave sizes in \pgf@xb and \pgf@yb
\newcommand*{\blockdiagramshape@sinewave}{
	\pgfpathsine{\pgfqpoint{\pgf@xb}{\pgf@yb}}
	\pgfpathcosine{\pgfqpoint{\pgf@xb}{-\pgf@yb}}
	\pgfpathsine{\pgfqpoint{\pgf@xb}{-\pgf@yb}}
	\pgfpathcosine{\pgfqpoint{\pgf@xb}{\pgf@yb}}
}%
\newcommand*{\blockdiagramshape@waveat}[2]{ %% wave \waveat{x,y}, coordinates in wave size
	\centerpoint
	\advance \pgf@x by #1\pgf@xb
	\advance \pgf@y by #2\pgf@yb
	\advance \pgf@x by -2\pgf@xb %% because \sinewave starts left
	\pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
	\blockdiagramshape@sinewave
}%
\newcommand*{\blockdiagramshape@strikeat}[2]{ %% strike through \strikeat{x,y}, coordinates in wave size
	\centerpoint
	\advance \pgf@x by .5\pgf@xb
	\advance \pgf@y by \pgf@yb
	\advance \pgf@x by #1\pgf@xb
	\advance \pgf@y by #2\pgf@yb
	\pgfpathmoveto{\pgfpoint{\pgf@x}{\pgf@y}}
	\centerpoint
	\advance \pgf@x by -.5\pgf@xb
	\advance \pgf@y by -\pgf@yb
	\advance \pgf@x by #1\pgf@xb
	\advance \pgf@y by #2\pgf@yb
	\pgfpathlineto{\pgfpoint{\pgf@x}{\pgf@y}}
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Bandpass
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{bandpass/.style={bandpassshape,operatorbox,sign scale/.initial=0.4}}%
\pgfdeclareshape{bandpassshape}{
	%% by SZ 2014-11
	\inheritsavedanchors[from=simplerect] %% has to be before \saveddimen
	\saveddimen\width{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=simplerect]
	\inheritanchors[from=simplerect]
	\inheritbackgroundpath[from=simplerect]
	%% Inner path:
	\beforebackgroundpath{
		\pgfmathsetlength{\pgfutil@tempdimb}{\pgfkeysvalueof{/tikz/sign scale}*\width}%% Size of sign
		%
		%% B: Offsets (wavelength, amplitude):
		\pgf@xb=\pgfutil@tempdimb %% half "wavelength"
		\divide \pgf@xb by 2
		\pgf@yb=\pgfutil@tempdimb %% amplitude
		\divide \pgf@yb by 3 %% lower than in "sineshape"
		%% center wave:
		\blockdiagramshape@waveat{0}{0}
		%% upper wave:
		\blockdiagramshape@waveat{0}{4}
		\blockdiagramshape@strikeat{0}{4}
		%% lower wave:
		\blockdiagramshape@waveat{0}{-4}
		\blockdiagramshape@strikeat{0}{-4}
		%% paint:
		\pgfusepathqstroke%
	}
	\nodeparts{} %% no text
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Highpass
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{highpass/.style={highpassshape,operatorbox,sign scale/.initial=0.5}}%
\pgfdeclareshape{highpassshape}{
	%% by SZ 2014-11
	\inheritsavedanchors[from=simplerect] %% has to be before \saveddimen
	\saveddimen\width{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=simplerect]
	\inheritanchors[from=simplerect]
	\inheritbackgroundpath[from=simplerect]
	%% Inner path:
	\beforebackgroundpath{
		\pgfmathsetlength{\pgfutil@tempdimb}{\pgfkeysvalueof{/tikz/sign scale}*\width}%% Size of sign
		%
		%% B: Offsets (wavelength, amplitude):
		\pgf@xb=\pgfutil@tempdimb %% half "wavelength"
		\divide \pgf@xb by 2
		\pgf@yb=\pgfutil@tempdimb %% amplitude
		\divide \pgf@yb by 3 %% lower than in "sineshape"
		%% upper wave:
		\blockdiagramshape@waveat{0}{2}
		%% lower wave:
		\blockdiagramshape@waveat{0}{-2}
		\blockdiagramshape@strikeat{0}{-2}
		%% paint:
		\pgfusepathqstroke%
	}
	\nodeparts{} %% no text
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Lowpass
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\tikzset{lowpass/.style={lowpassshape,operatorbox,sign scale/.initial=0.5}}%
\pgfdeclareshape{lowpassshape}{
	%% by SZ 2014-11
	\inheritsavedanchors[from=simplerect] %% has to be before \saveddimen
	\saveddimen\width{%
		%\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/radius}}%% does not work
		\pgfmathsetlength\pgf@x{\pgfkeysvalueof{/tikz/width}}
		\divide\pgf@x by 2
	}
	\inheritanchorborder[from=simplerect]
	\inheritanchors[from=simplerect]
	\inheritbackgroundpath[from=simplerect]
	%% Inner path:
	\beforebackgroundpath{
		\pgfmathsetlength{\pgfutil@tempdimb}{\pgfkeysvalueof{/tikz/sign scale}*\width}%% Size of sign
		%
		%% B: Offsets (wavelength, amplitude):
		\pgf@xb=\pgfutil@tempdimb %% half "wavelength"
		\divide \pgf@xb by 2
		\pgf@yb=\pgfutil@tempdimb %% amplitude
		\divide \pgf@yb by 3 %% lower than in "sineshape"
		%% upper wave:
		\blockdiagramshape@waveat{0}{2}
		\blockdiagramshape@strikeat{0}{2}
		%% lower wave:
		\blockdiagramshape@waveat{0}{-2}
		%% paint:
		\pgfusepathqstroke%
	}
	\nodeparts{} %% no text
}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Delay and Multiplexer blocks
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Alternatives for minimum height and minimum width, needed for multiplexer:
\tikzset{%
	%% http://tex.stackexchange.com/a/196845/50960
	%% Declare alternatives for minimum width and height that use the coordinate system units (x and y specified in \begin{tikzpicture}[x=...,y=...]
	%% (Only advisable when x and y are orthogonal)
	minimum width cs/.code={%
		\pgfpointxy{#1}{0}%
		\tikzset{minimum width/.expanded=\the\csname pgf@x\endcsname}%
	},
	minimum height cs/.code={%
		\pgfpointxy{0}{#1}%
		\tikzset{minimum height/.expanded=\the\csname pgf@y\endcsname}%
	},
}%
%% Delay block: (usage: \node [delay] {T or $z^{-1}$};)
\tikzset{delay/.style={draw,fill=white,minimum width=7mm,minimum height=7mm}}%
%% Multiplexer block: (usage: [mux=<height in tikzpicture y units>])
\tikzset{mux/.style={draw, fill, inner sep=0, minimum width=1mm, minimum height cs=#1}}%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Amplifier (just a triangle with useful anchors)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% amplifier
\tikzset{amplifier/.style={
		triangle,
		line join=round,
		operatorbox,
		%text depth=,text height=,%% undo these settings from [iks block]
		minimum width=0,
		minimum height=0,
	}
}%
\pgfdeclareshape{triangle}{
	%% by SZ 2018-07
	
	\saveddimen\width{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}%
		\pgf@x=\pgf@xa%
	}
	\saveddimen\halfwidth{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}%
		\pgf@x=\pgf@xa%
		\divide \pgf@x by 2
	}
	\saveddimen\height{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}%
		%% height = 2/√3 · width ⇒ gleichseitiges Dreieck
		\pgf@x=\pgf@xa%
		\multiply \pgf@x by 115
		\divide \pgf@x by 100
	}
	\saveddimen\halfheight{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}%
		\pgf@x=\pgf@xa%
		\multiply \pgf@x by 115
		\divide \pgf@x by 200
	}
	\saveddimen\quarterheight{
		\pgfmathsetlength{\pgf@xa}{\pgfkeysvalueof{/tikz/width}}%
		\pgf@x=\pgf@xa%
		\multiply \pgf@x by 115
		\divide \pgf@x by 400
	}
	
	
	\savedanchor\centerpoint{%
		\pgf@x=0pt%
		\pgf@y=0pt%
	}
	
	\anchor{text}{
		%% This looks somehow centered for some texts... but it's not really correct
		\centerpoint
		\advance\pgf@y by -0.5\ht\pgfnodeparttextbox
		\advance\pgf@y by \dp\pgfnodeparttextbox
		\advance\pgf@x by -0.5\wd\pgfnodeparttextbox
	}
	
	
	\anchor{base}{\centerpoint}
	\anchor{center}{\centerpoint}%% TODO: actually this should be moved to LOOK more like the center
	\anchor{north}{\centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by \halfheight}
	\anchor{south}{\centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by -\halfheight}
	\anchor{west}{\centerpoint \advance\pgf@x by -\halfwidth}
	\anchor{east}{\centerpoint \advance\pgf@x by \halfwidth}
	\anchor{north west}{\centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by \quarterheight}
	\anchor{south west}{\centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by -\quarterheight}
	\anchor{north east}{\centerpoint \advance\pgf@y by \quarterheight}
	\anchor{south east}{\centerpoint \advance\pgf@y by -\quarterheight}
	
	% 	%% Other: %% TODO (this was just copied from simplerect)
	% \anchorborder{\centerpoint} %% Currently it has to be specified manually
	\anchorborder{\centerpoint \advance\pgf@x by -\halfwidth} %% As long as it is not implemented, just connect to the "west" anchor
	\anchorborder{%% from pgfmoduleshapes.code.tex
		\pgf@xb=\pgf@x% xb/yb is target
		\pgf@yb=\pgf@y%
		%% If right from east: use east
		%% If neither left nor right: use north east or south east
		%% If left from west: Use west between north west and south west, and those if above or below
		%
		%% TODO: something is wrong here! The comparisons don't really work.
		%
		\centerpoint \advance\pgf@x by \halfwidth %% east
		\ifdim\pgf@xb<\pgf@x %% if not: the correct point is east, which is already chosen
			%% this means: the point is left of the east coordinate
			\centerpoint \advance\pgf@x by -\halfwidth %% west
			\ifdim\pgf@xb<\pgf@x %% point is left of west
				% \centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by \halfheight %% north west
				% %\PackageWarning{none}{point: \the\pgf@xb, \the\pgf@yb compared with: \the\pgf@x,  \the\pgf@y}
				% \ifdim\pgf@yb<\pgf@y %% lower than north west
				% 	\centerpoint \advance\pgf@x by -\halfwidth \advance\pgf@y by -\halfheight %% south west
				% 	\ifdim\pgf@yb>\pgf@y %% higher than south west
						\centerpoint \advance\pgf@x by -\halfwidth %% west
				% 	\else
				% 		%% south west is already selected: what we wanted
				% 	\fi
				% \else
				% 	%% north west is already selected: what we wanted
				% 	\PackageWarning{none}{test}
				% \fi
			\else %% point is right of west, i.e., inside the triangle (in x direction)
				\ifdim\pgf@yb>\pgf@y %% above center:
					\centerpoint \advance\pgf@y by \halfheight %% north east
				\else
					\centerpoint \advance\pgf@y by -\halfheight %% south east
				\fi
			\fi
		\fi
		%
	% 	% \southwest%
	% 	% \pgf@xa=\pgf@x% xa/ya is se
	% 	% \pgf@ya=\pgf@y%
	% 	%% south west:
	% 	\centerpoint
	% 	\pgf@xa=\pgf@x \advance\pgf@xa by -\halfwidth
	% 	\pgf@ya=\pgf@y \advance\pgf@ya by -\halfwidth
	% 	% \northeast%
	% 	\centerpoint \advance\pgf@y by \halfwidth \advance\pgf@x by \halfwidth %% north east
	% 	\advance\pgf@x by-\pgf@xa%
	% 	\advance\pgf@y by-\pgf@ya%
	% 	\pgf@xc=.5\pgf@x% x/y is half width/height
	% 	\pgf@yc=.5\pgf@y%
	% 	\advance\pgf@xa by\pgf@xc% xa/ya becomes center
	% 	\advance\pgf@ya by\pgf@yc%
	% 	\edef\pgf@marshal{%
	% 		\noexpand\pgfpointborderrectangle
	% 		{\noexpand\pgfqpoint{\the\pgf@xb}{\the\pgf@yb}}
	% 		{\noexpand\pgfqpoint{\the\pgf@xc}{\the\pgf@yc}}%
	% 	}%
	% 	\pgf@process{\pgf@marshal}%
	% 	\advance\pgf@x by\pgf@xa%
	% 	\advance\pgf@y by\pgf@ya%
	}
	
	\backgroundpath{
		%% get and set options
		\pgfutil@tempdima=\halfwidth
		
		%% Calculate points:
		\centerpoint
		%% south west:
		\pgf@xa=\pgf@x \advance\pgf@xa by -\halfwidth
		\pgf@ya=\pgf@y \advance\pgf@ya by -\halfheight
		%% north west:
		\pgf@xb=\pgf@x \advance\pgf@xb by -\halfwidth
		\pgf@yb=\pgf@y \advance\pgf@yb by \halfheight
		%% east:
		\pgf@xc=\pgf@x \advance\pgf@xc by \halfwidth
		\pgf@yc=\pgf@y %\advance\pgf@yc by \halfwidth
		
		
		%% Draw outer shape:
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc}}
		\pgfpathclose %% allow round corners
		
		%% Fill:
		% This is now done by the wrapper style
		\tikz@mode
		\iftikz@mode@fill
			\pgfusepath{draw,fill}
		\else
			\pgfusepath{draw}
		\fi
	}
}%
%
%
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Convolutional encoder
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Example usage:
% \begin{tikzpicture}[thick,
% 		x=1.5cm, %% x: horizontal distance between nodes
% 		y=1cm, %% y: vertical height of summation signs
% 	]
% 	%% Initialize:
% 	\draw (0,0) -- ++(0.5,0)
% 		coordinate [dot] (x0) coordinate (t0); %% don't care where. t0 is only for the edges
% 	\drawconvolutionalencoderbase[5] %% draw the delay blocks (constraint length 5)
% 	\draw [->] (mux.east) -- +(0.5,0); %% output
% 	%% Draw the polynomials:
% 	\drawconvolutionalcoefficients[x1]{1/3,2/4}
% 	\def\ypos{-1} %% draw below
% 	\drawconvolutionalcoefficients{1/1,2/3,3/4}
% \end{tikzpicture}
\newcommand*{\drawconvolutionalencoderbase}[1][\CL]{
	%% usage: \drawconvolutionalencoderbase[constraint length]
	%% (if constraint length is not given, use \CL)
	%% Coordinates (x0) and (t0) have to be defined before this e.g.:
	% \coordinate [dot] (x0) coordinate (t0); %% don't care where. t0 is only for the edges
	
	%% The coordinates (t#) are the #-th delay blocks
	%% The coordinates (x#) are the signal points after the #th delay block
	
	%% Make the chain of delays:
	\pgfmathtruncatemacro{\numnodes}{#1-1}
	\foreach \endnode in {1,...,\numnodes}{ %% Using endnode so we can start at 1
		\pgfmathtruncatemacro{\startnode}{\endnode-1}
		\path (x\startnode)
			++(0.5,0) node (t\endnode) [delay] {T} %% $z^{-1}$
			++(0.5,0) coordinate (x\endnode);
		\path (t\startnode) edge [->] (t\endnode);
	}
	\path (t\numnodes) edge [-] (x\numnodes);
	
	
	%% MUX:
	\path (x\numnodes) ++(0.75,0)
		%+(-0.5mm,-1.2) [fill] rectangle +(0.5mm,1.2);
		node (mux) [mux=2.5] {}; %2.5*\coeffheight
}%
\newcommand*{\drawconvolutionalcoefficients}[2][x0]{
	%% usage:
	% \drawconvolutionalcoefficients[coordinate of coeff0]{1/<coeff1>,2/<coeff2>,3/<coeff3>,...}
	
	\ifdefined\ypos\else\def\ypos{1}\fi %% \ypos should be set
	
	%% Polynomial ID:
	\ifdefined\p
		\pgfmathtruncatemacro{\p}{\p+1}
	\else
		\def\p{1}
	\fi
	
	%\pp: polynomial coefficient id
	%%\pos: position
	\coordinate (p_\p_0) at (#1); %% This is where the first addition will come from
	\foreach \pp/\pos in {#2} { %% First generator polynomial
		\pgfmathtruncatemacro{\lastpp}{\pp-1}
		\path (x\pos)
			node [dot] {}
			++(0,\ypos)
			node (p_\p_\pp) [sumbox] {}
			%% \p: polynomial id, \pp: polynomial coefficient id
			edge [<-] (x\pos)
		;
		\draw [->] (p_\p_\lastpp.east) |- (p_\p_\pp.west); %% east and west avoid a bug
		\global\edef\finalpp{\pp}
	}
	\draw [->] (p_\p_\finalpp.east) -- (p_\p_\finalpp.east-|mux.west);
}%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Wave front symbol
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Can be used in front of loudspeakers, antennas, 🔊, ...
%% Usage:
% \drawwavefronts	%% standard
% \drawwavefronts[thick,red,rotate=-30]	%% normal tikz styles can be used
% \drawwavefronts[opening angle=20,hide center,wave count=7,wave radius=1mm]	%% some custom styles
% \drawwavefronts[first wave=-2,wave count=5]	%% negative first wave for symmetrical symbol
\newcommand{\drawwavefronts}[1][]{%
	\tikz[
		baseline=(center),
		%% Define parameters:
		opening angle/.initial=60,
		wave count/.initial=3,
		first wave/.initial=1,
		wave radius/.initial=1ex,%% some value that scales with the font size
		wave front/.style={}, %% initialize
		center radius/.initial=0.5\pgflinewidth,
		center/.style={fill}, %% default
		draw center/.style={
			center/.append style={fill},
		},
		hide center/.style={
			center/.append style={fill=none},
		},
		%
		create bounding box/.code={%
			\def\wavefronts@boundingbox{}%
		},
		no bounding box/.code={%
			\let\wavefronts@boundingbox\undefined%
		},
		create bounding box,%% default: use the bounding box
		%% Default style to make it look pleasing:
		line cap=round, %% to reset to default: line cap=butt
		%% User-defined styles:
		#1, %% use optional parameters to change this function
	]{
		\pgfmathsetmacro{\wavefronts@startangle}{%
			(\pgfkeysvalueof{/tikz/opening angle})/2%
		}
		\pgfmathsetmacro{\wavefronts@endangle}{-(\wavefronts@startangle)}
		\def\wavenum{\pgfkeysvalueof{/tikz/wave count}}
		\def\radius{\pgfkeysvalueof{/tikz/wave radius}}
		\def\firstwave{\pgfkeysvalueof{/tikz/first wave}}
		\pgfmathsetmacro{\secondwave}{\firstwave+1}
		\pgfmathsetmacro{\lastwave}{\firstwave+\wavenum-1}
		\begin{pgfinterruptboundingbox}
			\foreach \thiswavenum in {\firstwave,\secondwave,...,\lastwave} {
				%\edef\thisradius{(\thiswavenum)*(\radius)}
				\draw [wave front]
					(\wavefronts@startangle:\thiswavenum*\radius) %% startpoint of the arc
					arc[
						radius=\thiswavenum*\radius,
						start angle=\wavefronts@startangle,
						end angle=\wavefronts@endangle,
					];
			}
			\path (0,0)
				coordinate (center)
				[center] circle (\pgfkeysvalueof{/tikz/center radius}) %% the center
				;
		\end{pgfinterruptboundingbox}
		\ifdefined\wavefronts@boundingbox %% user wants a bounding box: draw outer coordinates
			%% base/center:
			\path (0,0); %% TODO: only if it is shown(?)
			%% first wave (might be negative):
			\path (\wavefronts@startangle:\firstwave*\radius) arc[radius=\firstwave*\radius, start angle=\wavefronts@startangle, end angle=\wavefronts@endangle];
			%% last wave (usually the biggest:
			\path (\wavefronts@startangle:\lastwave*\radius) arc[radius=\lastwave*\radius, start angle=\wavefronts@startangle, end angle=\wavefronts@endangle];
		\fi
	}%
}%
